Non-blocking Patricia Tries with Replace Operations

This paper presents a non-blocking Patricia trie implementation for an asynchronous shared-memory system using Compare&Swap. The trie implements a linearizable set and supports three update operations: insert adds an element, delete removes an element and replace replaces one element by another. The replace operation is interesting because it changes two different locations of tree atomically. If all update operations modify different parts of the trie, they run completely concurrently. The implementation also supports a wait-free find operation, which only reads shared memory and never changes the data structure. Empirically, we compare our algorithms to some existing set implementations.

==> proof-query.tex <==
\subsection{Correctness of Query Operations} 
The find and rangeQuery operation are query operations.
In this section, we show how to linearize the query operations, if they return.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Correctness of the Find Operation}

Now, we show how to linearize find operations that terminate.
By Corollary \ref{search-val-in-trie-cor} and Lemma \ref{search-val-not-in-trie-lem}, we have the following corollaries.

\begin{corollary} \label{find-true-col}
If find($val$) returns true, a leaf node whose $label$ is $val$ is logically in the trie at some time during the find operation.
\end{corollary}

\begin{corollary}\label{find-false-col}
If find($val$) returns false, there is some time during the find operation when no leaf node whose $label$ is $val$ is logically in the trie.
\end{corollary}

The find operation is linearized at the time given by Corollary \ref{find-true-col} or \ref{find-false-col}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Correctness of the Predecessor Operation}
In this section, we show how to linearize the predecessor operations that terminate. 
%The comparing procedure of the predecessor operation begins at line \ref{begin-compare} and ends at line \ref{end-compare}.
%During the comparing procedure, the find nearest neighbour operation reads leaf nodes in $result$ at line \ref{nn-check} and internal nodes in $result$ at line \ref{nn-check}.
The operation calls the predecessorSearch routine at line \ref{pred-call-predSearch}. % just before the comparing procedure begins.
Assume predecessor($val$) terminates.
Let $T$ be the last execution of line \ref{pred-unmark1}, \ref{pred-unmark2} or \ref{pred-unmark3}. % and $T_2$ be the time when the last comparing procedure begins. 
We show that the operation can be linearized at $T$.
First, we have the definition of a predecessor.

\begin{definition}
Let $S$ be a non-empty set of values and $val$ be a value.
Then, $val'$ is a {\it predecessor} of $val$ among the values in $S$, if $val'$ is the greatest value in $S$ that is smaller than $val$. % dist($pt$, $pt'$) = min\{dist($pt$, $pt''$): $pt'' \in S$)\}.
\end{definition}

Now, we show if the operation returns, the $child$ fields that are in $result$ after the last call to predSearch returns have not been changed 
between the time when they are stored in $result$ and they are read at line \ref{pred-check-child}.

\begin{lemma} \label{pred-no-child-change-lem}
Assume predecessor($val$) returns.
Let $\langle node, child \rangle$ be an element in $result$ just after the last call to predSearch returns.
Then, $node.child = child$ at all times between the time 
when $\langle node, child \rangle$ is stored in $result$ at line \ref{predSearch-set-result1}, \ref{predSearch-set-result2} or \ref{predSearch-set-result3} and $node.child$ is read at line \ref{pred-check-child}.
\end{lemma}
\begin{proof}
Then, $child$ is the value of $node.child$ that is read at line  \ref{predSearch-set-result1}, \ref{predSearch-set-result2} or \ref{predSearch-set-result3}.
Since the operation returns just after the last call to predSearch, %$node.child$ that is read at line \ref{predSearch-set-result1}, \ref{predSearch-set-result2} or \ref{predSearch-set-result3} is the same as 
$node.child = child$ when it is read at line \ref{pred-check-child}.
By Lemma \ref{same-child-lem}, the lemma is true.
\end{proof}


By the pseudo-code, any node in $F_I - U_I$ is read from a $child$ field earlier by Lemma \ref{search-lem}.
An element of a $child$ field is set to a newly created node or an element of some $child$ field that is read earlier at line \ref{help-change-child}, \ref{create-copy}, \ref{create-internal}, \ref{mov-create-node1}, \ref{mov-create-node2} or \ref{mov-create-node3}. 
So, we have the following observation.
\begin{observation} \label{unmarked-root-obs}
The $root$ is never marked.
\end{observation}


??????Combine it with the next lemma??????
The following lemma shows that, after a node becomes reachable for the first time, if the node is unmarked, it is reachable. 
\begin{lemma} \label{marked-unreachable-lem}
Let $I$ be a Flag object. % and $x$ be an internal node in $F_I - U_I$.
Consider a child CAS of $I$ that succeeds at time $T$.
If $x$ becomes marked by $I$ just after $T$, $x$ is reachable immediately before $T$ and $x$ is unreachable immediately after $T$.
\end{lemma}
\begin{proof}
Let $I$ be a Flag object. 
Let $\langle gp$, $p$, $node$, -, -, $- \rangle$ be the result returned by the call to search($val$) on line \ref{ins-call-search}, \ref{del-call-search} or \ref{mov-call-search1} that precedes the creation of $I$.
If $I$ is created inside move($val$, $val'$), let $\langle$ -, $p'$, $node'$, -, -, $- \rangle$ be the result returned by the call to search($val'$) on line \ref{mov-call-search2} that precedes the creation of $I$.
We show that any node that becomes marked by $I$ just after $T$ becomes unreachable just after $T$.
We consider different cases according to what line created $I$.

Case 1: $I$ is created at line \ref{ins-set-info1}.
By Lemma \ref{search-lem} and Invariant \ref{prefix-lem}, $p \ne node$.
So, $node \in F_I - U_I$.
By the definition, $node$ is the only node that becomes marked by $I$ just after $T$.
Let $newNode$ be the new internal node whose non-empty children are a new leaf node and a new copy of $node$ at line \ref{ins-call-create-node}.
In this case, $I.oldChild[0] = node$ and $I.newChild[0] = newNode$.
%Since $node \in F_I$, by Lemma \ref{no-wrong-child-change-lem}, %$p.child$ is not changed between the time when $p.info$ is read for the last time during search($pt$) and $T$ and
%$node.child$ is not changed between the time when $node.info$ is read at line \ref{ins-read-node-info} and $T'$.
%Thus, just before $T'$, the $child$ field of the new copy of $node$ is the same as $node.child$.
%The only internal node that could become unreachable at $T'$ is $node$.
By Lemma \ref{search-lem}, $p$ is a parent of $node$ during the search operation.
Since $p \in F_I$ (by Observation \ref{reachable-parent-lem}), by Lemma \ref{no-wrong-child-change-lem}, $p$ is a parent of $node$ just before $T$.
By Lemma \ref{update-x-info-lem}, $p$ is not marked just before $T$.
Since $p$ is reachable at some time during the search operation (by Lemma \ref{query-reachable-lem}), $p$ is reachable just before $T$ (by Lemma \ref{unmarked-reachable-lem}).
So, by Lemma \ref{reachable-parent-lem}, $node$ is not a child of any other reachable node just before $T$.
Since the children of $newNode$ are a new leaf node and a new copy of $node$ just before $T$, $node$ is not a descendant of $newNode$ just before $T$ by Invariant \ref{prefix-inv}.
Since an element of $p.child$ is changed from $node$ to $newNode$ at $T$, $node$ is not reachable just after $T$. % since the children of $newNode$ are a new leaf node and a new copy of $node$.

Case 2: $I$ is created at line \ref{ins-set-info2} or \ref{mov-set-info-sc3}.
%Since the operation does not return at line \ref{} $I.oldChild[0]$ is a leaf node
Since $U_I = F_I$, no internal node would be marked by $I$ just after $T$ and the lemma is vacuously true.

Case 3: $I$ is created at line \ref{del-set-info1}.
By Lemma \ref{search-lem} and Invariant \ref{prefix-inv}, $gp \ne p$.
So, $p \in F_I - U_I$.
By the definition, $p$ is the only node that becomes marked by $I$ just after $T$.
Let $nodeSibling$ be an element of $p.child$ that is not $node$ at line \ref{del-read-sibling}.
By Invariant \ref{prefix-inv} and \ref{child-num-inv}, $nodeSibling \ne node$ exists.
In this case, $I.oldChild[0] = p$ and $I.newChild[0] = nodeSibling$.
By Lemma \ref{search-lem}, $gp$ is a parent of $p$ during the search operation.
Since $gp \in F_I$ (by Observation \ref{reachable-parent-lem}), by Lemma \ref{no-wrong-child-change-lem}, $gp$ is a parent of $p$ just before $T$.
By Lemma \ref{update-x-info-lem}, $gp$ is not marked just before $T$.
Since $gp$ is reachable at some time during the search operation (by Lemma \ref{query-reachable-lem}), $gp$ is reachable just before $T$ by Lemma \ref{unmarked-reachable-lem}.
So, by Lemma \ref{reachable-parent-lem}, $p$ is not a child of any other reachable node just before $T$.
Since $nodeSibling$ is a child of $p$ just before $T$ (by Lemma \ref{no-wrong-child-change-lem}), $p$ is not a descendant of $nodeSibling$ just before $T$ by Invariant \ref{prefix-inv}.
Since an element of $gp.child$ is changed from $p$ to $nodeSibling$ at $T$, $p$ is not reachable just after $T$ since $node \ne nodeSibling$.


Case 4: $I$ is created at line \ref{mov-set-info1} or \ref{mov-set-info2}.
%By Lemma \ref{search-lem} and Invariant \ref{correct-child-field-lem}, $p' \ne node'$.
%Since the conditions at line \ref{mov-check-gc-condition}, $gp \ne node'$.
%So, $node' \in U_I - F_I$.
If $T$ is the first CAS of $I$ on $I.pNode[0]$, since $I.oldChild[0] = node'$, if $node'$ is an internal node, by the definition, $node'$ is the only node that becomes marked by $I$ just after $T$.
By the same argument as Case 1, $node'$ becomes unreachable at $T$ if $node'$ is an internal node.
%By Lemma \ref{search-lem} and Invariant \ref{correct-child-field-lem}, $p \ne gp$.
%Since $p \ne p'$, $p \notin U_I$.
%By Corollary \ref{different-child-cas-col}, the child CAS of $I$ on $I.pNode[0]$ and $I.pNode[1]$ are on the different elements of the $child$ fields.
If $T$ is the first CAS of $I$ on $I.pNode[1]$, since $I.oldChild[1] = p$, by the definition, $p$ is the only node that becomes marked by $I$ just after $T$.
By the same argument to Case 3, $p$ becomes unreachable at $T$.


Case 5: $I$ is created at line \ref{mov-set-info-sc1}.
Then, $node'$ is an internal node and $p = p'$.
Since the condition at line \ref{mov-check-gc-condition}, $gp \ne node'$.
So, $node' \in F_I - U_I$.
By Lemma \ref{search-lem} and Invariant \ref{prefix-inv}, $p \ne gp$.
So, $p \in F_I - U_I$.
By the definition, $p$ and $node_i$ are the only nodes that become marked by $I$ just after $T$.
Let $newNode$ be the new internal node whose non-empty children are a new leaf node and a new copy of $node$ at line \ref{mov-call-create-node}.
In this case, $I.oldChild[0] = p$ and $I.newChild[0] = newNode$.
By Lemma \ref{search-lem}, $gp$ is a parent of $p$ during the search operation and $p$ is a parent of $node'$ during the search operation since $p = p'$.
Since $gp \in F_I$ (by Observation \ref{reachable-parent-lem}), by Lemma \ref{no-wrong-child-change-lem}, $gp$ is a parent of $p$ just before $T$ and $p$ is a parent of $node'$ just before $T$.
By Lemma \ref{update-x-info-lem}, $gp$ is not marked just before $T$ and $p$ is not marked just before $T$.
Since $gp$ is reachable at some time during the search operation (by Lemma \ref{query-reachable-lem}), $gp$ is reachable just before $T$ by Lemma \ref{unmarked-reachable-lem}.
Since $gp$ is reachable just before $T$ and $gp$ is a parent of $p$ just before $T$, $p$ is reachable just before $T$.
So, by Lemma \ref{reachable-parent-lem}, $p$ is not a child of any other reachable node just before $T$ and $node$ is not a child of any other reachable node just before $T$.
Since the children of $newNode$ are a new leaf node and a new copy of $node$ just before $T$, $node$ is not a descendant of $newNode$ just before $T$ by Invariant \ref{prefix-inv}.
Since an element of $gp.child$ is changed from $p$ to $newNode$ at $T$, $p$ and $node$ are not reachable just after $T$. % since the children of $newNode$ are a new leaf node and a new copy of $node$.



Case 6: $I$ is created at line \ref{mov-set-info-sc2}.
Then, $node'$ is a leaf node and $p = p'$.
By Lemma \ref{search-lem} and Invariant \ref{prefix-inv}, $p \ne gp$.
So, $p \in F_I - U_I$.
By the definition, $p$ is the only node that becomes marked by $I$ just after $T$.
Let $newNode$ be the new internal node whose non-empty children are a new leaf node and a new copy of $node$ at line \ref{mov-call-create-node}.
In this case, $I.oldChild[0] = p$ and $I.newChild[0] = newNode$.
By Lemma \ref{search-lem}, $gp$ is a parent of $p$ during the search operation.
Since $gp \in F_I$ (by Observation \ref{reachable-parent-lem}), by Lemma \ref{no-wrong-child-change-lem}, $gp$ is a parent of $p$ just before $T$.
By Lemma \ref{update-x-info-lem}, $gp$ is not marked just before $T$.
Since $gp$ is reachable at some time during the search operation (by Lemma \ref{query-reachable-lem}), $gp$ is reachable just before $T$ by Lemma \ref{unmarked-reachable-lem}.
So, by Lemma \ref{reachable-parent-lem}, $p$ is not a child of any other reachable node just before $T$.
Since the children of $newNode$ are a new leaf node and a new copy of $node$ just before $T$, $node$ is not a descendant of $newNode$ just before $T$ by Invariant \ref{prefix-inv}.
Since an element of $gp.child$ is changed from $p$ to $newNode$, $p$ is not reachable just after $T$. % since the children of $newNode$ are a new leaf node and a new copy of $node$.


Case 7: $I$ is created at line \ref{mov-set-info-sc4}.
By Lemma \ref{search-lem} and Invariant \ref{correct-child-field-lem}, $gp \ne p$.
So, $p \in F_I - U_I$.
By the definition, $p$ is the only node that becomes marked by $I$ just after $T$.
Let $nodeSibling$ be an element of $p.child$ that is not $node$ at line \ref{mov-read-sibling}.
By Invariant \ref{prefix-inv} and \ref{child-num-inv}, $nodeSibling \ne node$ exists.
Let $newNode$ be the new internal node whose non-empty children are a new leaf node and $nodeSibling$ at line \ref{mov-create-node1}.
In this case, $I.oldChild[0] = p$ and $I.newChild[0] = newNode$.
%First, we show $gp = p'$.
%By Lemma \ref{search-lem} and \ref{no-wrong-child-change-lem}, $gp.child[gpPos] = p$ at all times between the last time $gp.info$ is read during the search operation that is called at line \ref{mov-call-search1} and $T$.
%By Lemma \ref{query-reachable-lem}, $gp$ is reachable at some time during the search operation that is called at line \ref{mov-call-search1} and $T$.
%Since $gp.info=I$ just before $T$ (by Corollary \ref{flag-node-before-child-cas-col}) and $gp \notin F_I - U_I$, $gp$ is reachable just before $T$ by Lemma \ref{unreachable-mark-lem}.
%By Lemma \ref{no-reachable-after-unreachable-lem}, $gp$ is reachable at all times between the search operation that is called at line \ref{mov-call-search1} returns and $T$.
%By Lemma \ref{query-reachable-lem}, $p'$ is reachable and a parent of $node'$ at some time during the search operation that is called at line \ref{mov-call-search2}.
%Since $node' = p$, $gp$ and $p'$ are reachable parents of $node' = p$ at the same time during the search operation that is called at line \ref{mov-call-search2}.
%By Invariant \ref{correct-child-field-lem}, $gp = p'$ and $gpPos = pPos'$.
By Lemma \ref{search-lem}, $gp$ is a parent of $p$ during the search operation.
Since $gp \in F_I$ (by Observation \ref{reachable-parent-lem}), by Lemma \ref{no-wrong-child-change-lem}, $gp$ is a parent of $p$ just before $T$.
By Lemma \ref{update-x-info-lem}, $gp$ is not marked just before $T$.
Since $gp$ is reachable at some time during the search operation (by Lemma \ref{query-reachable-lem}), $gp$ is reachable just before $T$ by Lemma \ref{unmarked-reachable-lem}.
So, by Lemma \ref{reachable-parent-lem}, $p$ is not a child of any other reachable node just before $T$.

Since $nodeSibling$ is a child of $p$ just before $T$ (by Lemma \ref{no-wrong-child-change-lem}), $p$ is not a descendant of $nodeSibling$ just before $T$ by Invariant \ref{prefix-inv}.
Since the children of $newNode$ are a new leaf node and $nodeSibling$ just before $T$, % and $nodeSibling$ is a child of $p$ just before $T$ (by Lemma \ref{no-wrong-child-change-lem}), 
$p$ is not a descendant of $newNode$ just before $T$.
Since an element of $gp.child$ is changed from $p$ to $newNode$, $p$ is not reachable just after $T$.

Case 8: $I$ is created at line \ref{mov-set-info-sc5}.
Then, $gp = node'$.
By Lemma \ref{search-lem}, $gp$ was a parent of $p$ at some time during the search operation and $p'$ was a parent of $node' = gp$ at some time during the search operation.
By Invariant \ref{prefix-inv}, $gp \ne p'$ and $p \ne p'$.
So, $gp \in F_I - U_I$ and $p \in F_I - U_I$.
By the definition, $gp$ and $p$ are the only nodes that become marked by $I$ just after $T$.
Let $nodeSibling$ be an element of $p.child$ that is not $node$ at line \ref{mov-read-sibling} and $pSibling$ be an element of $gp.child$ that is not $p$ at line \ref{mov-create-node2}.
By Invariant \ref{prefix-inv} and \ref{child-num-inv}, $nodeSibling \ne node$ and $pSibling \ne p$ exist.
Let $nodeCopy$ be the new internal node whose non-empty children are $pSibling$ and $nodeSibling$ at line \ref{mov-create-node2} and 
$newNode$ be the new internal node whose non-empty children are a new leaf node and $nodeCopy$ at line \ref{mov-create-node1}.
In this case, $I.oldChild[0] = node'$ and $I.newChild[0] = newNode$.
By Lemma \ref{search-lem}, $p'$ is a parent of $node' = gp$ during the search operation and $gp$ is a parent of $p$ during the search operation since $gp = node'$.
Since $p' \in F_I$ (by Observation \ref{reachable-parent-lem}), by Lemma \ref{no-wrong-child-change-lem}, $p'$ is a parent of $node' = gp$ just before $T$ and $gp$ is a parent of $p$ just before $T$.
By Lemma \ref{update-x-info-lem}, $p'$ is not marked just before $T$ and $gp$ is not marked just before $T$.
Since $p'$ is reachable at some time during the search operation (by Lemma \ref{query-reachable-lem}), $p'$ is reachable just before $T$ by Lemma \ref{unmarked-reachable-lem}.
Since $p'$ is reachable just before $T$ and $p'$ is a parent of $node' = gp$ just before $T$, $gp$ is reachable just before $T$.
So, by Lemma \ref{reachable-parent-lem}, $gp$ is not a child of any other reachable node just before $T$ and $p$ is not a child of any other reachable node just before $T$.

Since $nodeSibling$ is a child of $p$ just before $T$ and $p$ is a child of $gp$ just before $T$ (by Lemma \ref{no-wrong-child-change-lem}), 
$p$ and $gp$ are not a descendant of $nodeSibling$ just before $T$ by Invariant \ref{prefix-inv}.
Since $pSibling$ and $p$ are children of $gp$ just before $T$ (by Lemma \ref{no-wrong-child-change-lem}), 
$p$ and $gp$ is not a descendant of $pSibling$ just before $T$ by Invariant \ref{prefix-inv}.
Since the children of $newNode$ are a new leaf node and $nodeCopy$ and the children of $nodeCopy$ are $nodeSibling$ and $pSibling$ just before $T$,
$gp$ and $p$ are not a descendant of $newNode$ just before $T$.
Since an element of $p'.child$ is changed from $node' = gp$ to $newNode$ at $T$, $gp$ and $p$ are not reachable just after $T$.
\end{proof}



??? COMPLETE THE PROOF
\begin{lemma}
If isMarked($node$, $nodeInfo$) returns true at $T$, $node$ is marked at $T$, otherwise $node$ is unmarked at $T$.
\end{lemma}
\begin{proof}
Let $I$ be a Flag object.
If $I.pNode$ has one element, after the first child CAS of $I$, any node in $F_I - U_I$ is marked by $I$.
Otherwise, if $I.oldChild[0]$ is an internal node, $I.oldChild[0]$ is marked by $I$ after the first child CAS of $I$ on $I.pNode[0]$ and 
$I.oldChild[1]$ is marked by $I$ after the first child CAS of $I$ on $I.pNode[1]$.

First, we show $node$ is marked at $T$ if isMarked($node$, $nodeInfo$) returns true at $T$.

Suppose $I.pNode$ has one element.
Since isMarked returns true, $nodeInfo$ is a Flag object $I$.
If the operation returns true at line \ref{isMarked-return-false1}, then $node \notin U_I$, $I.flagDone$ is true and $I.oldChild[0]$ is not in $I.pNode[0].child$.

Then, the $info$ field of any node in $F_I - U_I$ is $I$ at all times after the first child CAS of $I$ 
by Lemma \ref{change-child-after-flag-lem}, \ref{no-unflag-before-first-change-child-lem} and \ref{no-backtrack-after-first-change-child-lem}.
\end{proof}

Next, we show if the operation returns a leaf node, the leaf node is logically in the trie at~$T$.
\begin{lemma} \label{pred-leaf-in-trie-lem}
Assume predecessor($val$) returns $predLeaf$ at line \ref{predSearch-return1} or \ref{predSearch-return3}.
Then, $predLeaf$ is logically in the trie at $T$. 
\end{lemma}
\begin{proof}
Since $node$ is initially set to $root$ at line \ref{predSearch-set-initial-node} and an element of a $child$ field is not null by Invariant \ref{child-num-inv}, 
$node$ does not set to null at line \ref{predSearch-visit-node1}, \ref{predSearch-visit-node2} or \ref{predSearch-visit-node3}.
Thus, $predLeaf$ is not null.

First, we show $predLeaf$ is not logically removed at $T$.
Since the operation returns at line \ref{pred-return}, $predLeaf$ is not logically removed at the last execution of line \ref{pred-check-log-removed} (by Lemma \ref{logically-remove-lem}).
%By Lemma \ref{query-reachable-lem}, $predLeaf$ is reachable at some time during the last call to the predSearch.
So, by the definition, $predLeaf$ is not logically removed at $T$ before the last execution of line \ref{pred-check-log-removed}.
Next, we show that $predLeaf$ is reachable at $T$.

Let $result_T$ be the value of $result$ just after $T$.
Let $anc$ be the lowest internal node in $result_T$ that is unmarked at $T$ and whose $label$ is a prefix of $predLeaf.label$.
By Invariant \ref{prefix-inv}, $(anc.label) \cdot i$ is a prefix of $predLeaf.label$ for some $i$.
First, we show that $anc$ exists and $anc.child[i]$ is visited during the last call to the predSearch.
We consider different cases according to what line of the predSearch returns.

Case 1: The operation returns at line \ref{predSearch-return1}. 
Then, $predLeaf$ is read at line \ref{predSearch-visit-node1} and nodes are stored in $result$ only at line \ref{predSearch-set-result1}.
So,  the $label$ of any node that is saved in $result$ during the last call to the predSearch is a prefix of $predLeaf.label$ (by Invariant \ref{prefix-inv}).
Since $root$ is never marked (by Observation \ref{unmarked-root-obs}) and $\langle root, root.child \rangle$ is saved in $result$ at the first execution of line \ref{predSearch-set-result1}, 
$result_T$ is not empty and $anc$ exists.
So, $anc$ and $ancChild[i]$ are visited at line \ref{predSearch-visit-node1} (by Invariant \ref{prefix-inv}).

Case 2:  The operation returns at line \ref{predSearch-return3}.
Then, $predLeaf$ is read at line \ref{predSearch-visit-node2} or \ref{predSearch-visit-node3}.
Let $xPredAnc$ be the value of $predAnc$ at line \ref{predSearch-check-internal}.
So, either $predAnc$ is set to $xPredAnc$ at line \ref{predSearch-set-predAnc2} or at the last execution of line \ref{predSearch-set-predAnc1} (since the operation does not return at line \ref{predSearch-return2}).
%Since the operation does not return at line \ref{predSearch-return2}, $xPredAnc$ is not null and $predAnc$ is set to $xPredAnc$ at the last execution of line \ref{predSearch-set-predAnc1}.
If $node$ is not set at line \ref{predSearch-visit-node2}, the $label$ of any node that is stored in $result$ at line \ref{predSearch-set-result1} or \ref{predSearch-set-result3} is 
a prefix of $predLeaf.label$ (by Invariant \ref{prefix-inv}).
Otherwise, $xPredAnc.label$ and the $label$ of any node that is stored in $result$ at line \ref{predSearch-set-result} before $xPredAnc$ or at line \ref{predSearch-set-result3} is 
a prefix of $predLeaf.label$ (by Invariant \ref{prefix-inv}).
%Since $predLeaf = xPredAnc.child[0]$, $xPredAnc.label$ and the $label$ of any node that is visited at line \ref{predSearch-visit-node1} before $xPredAnc$ or 
%at line \ref{predSearch-set-result2} is a prefix of $predLeaf.label$ (by Invariant \ref{prefix-inv}).
%So, $xPredAnc.label$ and the $label$ of any node that is stored at line \ref{predSearch-set-result1} before $xPredAnc$ or at line \ref{predSearch-set-result2} is a prefix of $predLeaf.label$.
Since $root$ is never marked (by Observation \ref{unmarked-root-obs}) and $\langle root, root.child \rangle$ is saved in $result$ at the first execution of line \ref{predSearch-set-result1}, 
$result_T$ is not empty and $anc$ exists.
If $node$ is not set at line \ref{predSearch-visit-node2}, $anc$ and $anc.child[i]$ is visited at line \ref{predSearch-visit-node1} or \ref{predSearch-visit-node3} (by Invariant \ref{prefix-inv}).
Otherwise, If $anc$ is visited at line \ref{predSearch-visit-node1} before $xPredAnc$ or at line \ref{predSearch-visit-node3}, 
$anc.child[i]$ is visited at line \ref{predSearch-visit-node1} or \ref{predSearch-visit-node3} (by Invariant \ref{prefix-inv}). 
%Thus, $anc$ is either $xPredAnc$ or visited before $xPredAnc$.
If $node$ is not set at line \ref{predSearch-visit-node2} and $anc = xPredAnc$, $anc.child[i]$ is visited at line \ref{predSearch-visit-node2}. 

Let $ancChild$ be $anc.child[i]$ that is visited.
Since $anc$ and $anc.child[i]$ are visited during the last call of the predSearch, $anc$ and $ancChild$ are stored in $result$.
Since $anc$ is in $result_T$ and $ancChild$ is visited after $T$, $ancChild$ is in $result_T$. 
So, $anc.child[i] = ancChild$ at $T$ (by Lemma \ref{pred-no-child-change-lem}).

Now, we show that $predLeaf$ is reachable at $T$.
%Then, $anc.label$ is a prefix of $predLeaf.label$.
By Lemma \ref{unmarked-reachable-lem} and \ref{query-reachable-lem}, $anc$ is reachable at $T$. 
%By Lemma \ref{pred-no-child-change-lem}, $anc.child[i] = ancChild$ at $T$.
If $ancChild$ is a Leaf node, since $(anc.label) \cdot i$ is a prefix of $predLeaf.label$ and $predLeaf$ is visited earlier, $ancChild = predLeaf$.
Since $anc.child[i] = ancChild$ at $T$ and $anc$ is reachable at $T$, $ancChild = predLeaf$ is reachable at $T$.

Now, we show $predLeaf$ is reachable at $T$ if $ancChild$ is an Internal node.
To derive a contradiction, assume $predLeaf$ is not reachable at $T$.
%Since $ancChild$ is visited earlier, $ancChild$ is stored in $result$. % during the last call to the predSearch.
%Since $anc$ is in $result$ just after $T$, $ancChild$ is in $result$ just after $T$. % if $ancChild$ is an internal node.
Since $anc$ is reachable at $T$ and $anc.child[i] = ancChild$ at $T$, $ancChild$ is reachable at $T$. 
By Lemma \ref{marked-unreachable-lem}, $ancChild$ is unmarked at $T$. % if $ancChild$ is an internal node.
Since $ancChild$ is in $result_T$ and $ancChild$ is unmarked at $T$, $ancChild.label$ is not a prefix of $predLeaf.label$ by the definition of $anc$.
Then, $ancChild$ is not read at line \ref{predSearch-visit-node2} or \ref{predSearch-visit-node3} by Invariant \ref{prefix-inv}.
If $node$ is not set at line \ref{predSearch-visit-node2}, the $label$ of any node that is stored in $result$ at line \ref{predSearch-set-result1}, \ref{predSearch-set-result2} or \ref{predSearch-set-result3} is 
a prefix of $predLeaf$ (by Invariant \ref{pref-x-inv}).
So, $node$ is set at line \ref{predSearch-visit-node2}.
Since $xPredAnc.child[0]$ is visited at line \ref{predSearch-visit-node}, $(anc.label) \cdot 0$ is a prefix of $predLeaf.label$.
So, $xPredAnc.label$ or the $label$ of any node that is visited at line \ref{predSearch-visit-node1} before $sPredAnc$ is a prefix of $predLeaf.label$ and 
$xPredAnc.child[1].label$ is not a prefix of $predLeaf.label$ (by Invariant \ref{prefix-inv}).
Since $ancChild.label$ is not a prefix of $predLeaf.label$ and $anc.label$ is a prefix of $predLeaf.label$, $anc = xPredAnc$, $ancChild$ was read from $xPredAnc.child[1]$ and $i=1$,
%So, $xPredAnc.child[0]$ is visited at line \ref{predSearch-visit-node2}  $xPredAnc.child[0].label$ is a prefix of $predLeaf.label$ and $i = 0$
contradicting the fact that $(anc.label) \cdot i$ is a prefix of $predLeaf.label$.
\end{proof}

\begin{comment}
Let $I$ be a Flag object.
Let $\langle -$, -, $node_d$, -, -, $-\rangle$ be the result returned by the call to the search operation on line \ref{mov-call-search1} that precedes the creation of $I$ and
$\langle$-, -, $node_i$, -, -, $-\rangle$ be the result returned by the call to the search operation on line \ref{mov-call-search2} that precedes the creation of $I$.
IF $I$ is created at line \ref{mov-set-info-sc3}, since $node_i = node_d$ and the operation is not return at line \ref{mov-return-false1}, $node_i = node_d$ is a leaf node.
By the pseudo-code, we have the following observation.

\begin{obs} \label{old-child-obs}
Let $I$ be a Flag object.
Then, for each $i$, $I.oldChild[i] \in F_I - U_I$.
\end{obs}
\end{comment}

Now, we show the operation returns the correct node as a predecessor among the leaf nodes that are reachable at $T$ according the definition of the predecessor.
\begin{lemma} \label{pred-leaf-not-in-trie1-lem}
If predecessor($val$) returns null at line \ref{predSearch-return2}, each leaf node that is logically in the trie at $T$ does not contain a $label$ that is less than $val$.
\end{lemma}
\begin{proof}
%First, assume predecessor($val$) returns null.
To derive a contradiction, assume that a leaf node $leaf$ is logically in the trie at $T$ whose $label$ is less than $val$.
Let $result_T$ be the value of $result$ just after $T$.
Let $anc$ be the lowest internal node in $result_T$ whose $label$ does not include any $1$-bit and that is unmarked at $T$. % and visited earlier at line \ref{predSearch-visit-node1} during the last call to the predSearch.
Since $root$ is never marked (by Observation \ref{unmarked-root-obs}), $root.label = \varepsilon$ and $\langle root, root.child \rangle$ is saved in $result$ at the first execution of line \ref{predSearch-set-result1}, 
$result_T$ is not empty and $anc$ exists. 
%Since $anc$ was visited at line \ref{predSearch-visit-node1} earlier than $xNode$ was visited at line \ref{predSearch-visit-node1}, $anc.label$ is a prefix of $xNode.label$ (by Invariant \ref{prefix-inv}).
By Lemma \ref{unmarked-reachable-lem} and \ref{query-reachable-lem}, $anc$ is reachable at $T$. 
First, we show $anc$ is an ancestor of $leaf$ at $T$.

To derive a contradiction, assume $anc$ is not an ancestor of $leaf$ at $T$.
Since both $leaf$ and $anc$ are reachable at $T$ and $anc$ is not an ancestor of $leaf$ at $T$, $anc.label$ is not a prefix of $leaf.label$ (by Invariant \ref{prefix-inv}).
Let $i$ be the leftmost bit of $anc.label$ that is different from that bit of $leaf.label$.
Let $xNode$ be the node that is read at the last execution of line \ref{predSearch-visit-node1}. % during the last call to the predSearch.
If $xNode$ is a leaf node, $xNode.label \ge val$ since the operation does not return at line \ref{predSearch-return1}.
If $xNode$ is an internal node, $xNode.label$ is more than or equal to $|xNode.label|$ bits of $val$ since the operation satisfies the conditions at line \ref{predSearch-check-ancestor}.
%Since $anc$ is an ancestor of $node$ that is visited at line \ref{predSearch-visit-node1}, $anc.label$ is a prefix of $val$ since the condition at line \ref{predSearch-check-node} for $anc$ is satisfied.
Since $leaf.label < val$ by the assumption, $leaf.label$ is less than $xNode.label$ if $xNode$ is a leaf node or $|xNode.label|$ bits of $leaf.label$ is less than or equal to $xNode.label$ if $xNode$ is an internal node.
Since $i$ is the leftmost bit of $anc.label$ that is different from that bit of $leaf.label$ and $anc.label$ is a prefix of $xNode.label$, $i$th bit of $anc.label$ is not 0.
So, $i$th bit of $anc.label$ is 1, contradicting the fact that $anc.label$ does not include any $1$-bit.

%%%%%%%%%%%%%%%%
Thus, $anc$ is an ancestor of $leaf$ at $T$.
Since the operation returns null, the variable of $predAnc$ is not set at line \ref{predSearch-set-predAnc1} and the operation does not visit the element $child[1]$ of any node at line \ref{predSearch-visit-node1}.
Let $ancChild$ be $anc.child[0]$ when it is visited earlier at line \ref{predSearch-visit-node1} during the predSearch.
Since $anc.child[0]$ was $ancChild$ at line \ref{predSearch-visit-node1}, $(|anc.label| + 1)$th bit of $val$ is $0$.
Since $anc.label$ is a prefix of $leaf.label$ and $leaf.label$ is less than $val$, $(|anc.label| + 1)$th bit of $leaf.label$ is $0$.
By Lemma \ref{pred-no-child-change-lem}, $anc.child[0] = ancChild$ at $T$.
Since $anc$ is reachable at $T$, $ancChild$ is reachable at $T$.
By Lemma \ref{unreachable-flag-lem}, $ancChild$ is unmarked at $T$.
Since $anc$ is the lowest unmarked ancestor of $leaf$ at $T$, $ancChild$ is not an ancestor of $leaf$ at $T$.
Since $anc$ is visisted earlier at line \ref{predSearch-visit-node1}, $anc$ and $anc.child$ is stored in $result$ at line \ref{predSearch-set-result1}.
Since $anc$ is the lowest ancestor of $node$ that is unmarked at $T$, $anc$ is in $result$ when the operation returns.
Since $anc.child[0] = ancChild$ at $T$, $(|anc.label| + 1)$th bit of $leaf.label$ is $0$ and $ancChild$ is not ancestor of $leaf$ at $T$, $leaf$ is not reachable at $T$, contradicting that $leaf$ is logically in the trie at $T$.
\end{proof}


\begin{lemma} \label{pred-leaf-not-in-trie2-lem}
If predecessor($val$) returns $predLeaf$ at line \ref{predSearch-return1}, each leaf node that is logically in the trie at $T$ does not contain a $label$ that is less than $val$ and more than $predLeaf.label$.
\end{lemma}
\begin{proof}
To derive a contradiction, assume that a leaf node $leaf$ is logically in the trie at $T$ whose $label$ is more than $predLeaf.label$ and less than $val$.
Then, $predLeaf$ is the last node that is read at line \ref{predSearch-visit-node1} during the last call to the predSearch.
Let $anc$ be the lowest internal node that is unmarked at $T$ and visited earlier at line \ref{pred-visit-node1} during the last call to the predSearch.
(Since $root$ is never marked, such an ancestor exists at $T$.)
By Lemma \ref{unmarked-reachable-lem} and \ref{query-reachable-lem}, $anc$ is reachable at $T$. 
First, we show that $anc$ is an ancestor of $leaf$ at $T$. 

To derive a contradiction, assume $anc$ is not an ancestor of $leaf$ at $T$.
Since both $leaf$ and $anc$ are reachable at $T$, $anc.label$ is not a prefix of $leaf.label$.
Let $i$ be the leftmost bit of $anc.label$ that is different from that bit of $leaf.label$.
Since $anc$ was visited at line \ref{predSearch} earlier than $predLeaf$ was visited at line \ref{predSearch}, $anc.label$ is a prefix of $predLeaf.label$ by Invariant \ref{prefix-inv}. 
Since $predLeaf.label < leaf.label$ and $anc.label$ is a prefix of $predLeaf.label$, $i$th bit of $anc.label$ is 0.
Thus, $i$th bit of $leaf.label$ is 1.
Since the last node that is visited at line \ref{predSearch-visit-node1} is a leaf node, the condition at line \ref{predSearch-check-node} for $anc$ is satisfied.
So, $anc.label$ is a prefix of $val$.
Thus, $i$th bit of $val$ is 0, contradicting the fact that $leaf.label < val$ since $i$th bit of $leaf.label$ is 1. 

So, $anc$ is an ancestor of $leaf$ at $T$.
Let $ancChild$ be $anc.child[i]$ when it is visited earlier at line \ref{predSearch-visit-node1} during the predSearch.
If $i=0$, since $anc.label$ is a prefix of $leaf.label$ by Invariant \ref{prefix-inv} and $(anc.label) \cdot 0$ is a prefix of $val$ and $leaf.label < val$, $(|anc.label| + 1)$th bit of $val$ is $0$.
If $i=1$, since $anc.label$ is a prefix of $leaf.label$ by Invariant \ref{prefix-inv} and $(anc.label) \cdot 1$ is a prefix of $preLeaf.label$ by Invariant \ref{prefix-inv} and $predLeaf.label < leaf.label$, 
$(|anc.label| + 1)$th bit of $val$ is $1$.
Thus, $(anc.label) \cdot i$ is a prefix of $leaf.label$.
Since $anc$ is visisted earlier at line \ref{predSearch-visit-node1}, $anc$ and $anc.child$ is stored in $result$ at line \ref{predSearch-set-result1}.
Since $anc$ is the lowest internal node that is unmarked at $T$, $anc$ is in $result$ when the operation returns.
By Lemma \ref{pred-no-child-change-lem}, $anc.child[i] = ancChild$ at $T$.
Since $anc$ is reachable at $T$, $ancChild$ is reachable at $T$.
By Lemma \ref{unreachable-flag-lem}, $ancChild$ is unmarked at $T$.
Since $anc$ is the lowest unmarked ancestor of $leaf$ at $T$, $ancChild$ is not an ancestor of $leaf$ at $T$.
Since $anc.child[i] = ancChild$ at $T$, $(|anc.label| + 1)$th bit of $leaf.label$ is $i$ and $ancChild$ is not ancestor of $leaf$ at $T$, $leaf$ is not reachable at $T$, contradicting that $leaf$ is logically in the trie at $T$.
\end{proof}



\begin{lemma} \label{pred-leaf-not-in-trie3-lem}
If predecessor($val$) returns $predLeaf$ at line \ref{predSearch-return3}, each leaf node that is logically in the trie at $T$ does not contain a $label$ that is less than $val$ and more than $predLeaf.label$.
\end{lemma}
\begin{proof}
Let $node$ be the last node that is read at line \ref{predSearch-visit-node1} during the last call to the predSearch.
We consider different cases.

Case 1: $node$ is a Leaf node or $node$ is an Internal and  $node.label \ge |node.label|$ bits of $val$.
Let $predAnc$ is the node that is set at the last executin of line \ref{predSearch-set-predAnc1} during the last call to the predSearch.
Let $anc$ be the lowest internal node that is unmarked at $T$, whose $label$ is a prefix of $predAnc.label$ and visited earlier than at line \ref{predSearch-visit-node1} during the last call to the predSearch.
(Since $root$ is never marked, such an ancestor exists at $T$.)
By Lemma \ref{unmarked-reachable-lem} and \ref{query-reachable-lem}, $anc$ is reachable at $T$. 

First, we show $anc$ is an ancestor of $leaf$ at $T$.
To derive a contradiction, assume $anc$ is not an ancestor of $leaf$ at $T$.
Since both $leaf$ and $anc$ are reachable at $T$, $anc.label$ is not a prefix of $leaf.label$.
Let $i$ be the leftmost bit of $anc.label$ that is different from that bit of $leaf.label$.
Since $node$ is set to $predAnc.child[0]$ at line \ref{predSearch-visit-node2} before reading $predLeaf$ at line \ref{predSearch-visit-node2}, $predAnc.label$ is a prefix of $predLeaf.label$ by Invariant \ref{prefix-inv}.
Since $predLeaf.label < leaf.label$ and $anc.label$ is a prefix of $predLeaf.label$, $i$th bit of $anc.label$ is 0.
Thus, $i$th bit of $leaf.label$ is 1.
Since the last node that is visited at line \ref{predSearch-visit-node1} is a leaf node, the condition at line \ref{predSearch-check-node} for $anc$ is satisfied.
So, $anc.label$ is a prefix of $val$.
Thus, $i$th bit of $val$ is 0, contradicting the fact that $leaf.label < val$ since $i$th bit of $leaf.label$ is 1. 

So, $anc$ is an ancestor of $leaf$ at $T$.
Let $ancLeaf$ be the lowest internal node whose $label$ is a prefix of $leaf.label$ and that is unmarked at $T$ and visited at line \ref{predSearch-visit-node1}, \ref{predSearch-visit-node2} or \ref{predSearch-visit-node3}.
(Since $anc$ exists, such an ancestor of $leaf$ at $T$ exists.)
Let $ancChild$ be $ancLeaf.child[i]$ when it is visited earlier at line \ref{predSearch-visit-node1} during the predSearch.
%If $(|predAnc.label|+1)$th bit of $leaf.label$ is $0$, $ancLeaf$ is visited at line \ref{predSearch-visit-node1} after  $leaf.label < val$, 
%Then, $ancLeaf.label$ is a prefix of $predLeaf.label$ or $val$ or both.
Now, we show $(ancLeaf.label) \cdot i$ is a prefix of $leaf.label$.

If $ancLeaf$ is visited at line \ref{predSearch-visit-node1} before visiting $predAnc$ at line \ref{predSearch-visit-node1}, by Invariant \ref{prefix-inv},
since $predAnc.label$ is a prefix of both $val$ and $predLeaf.label$ and $(ancLeaf.label) \cdot i$ is a prefix of $predAnc.label$, $(ancLeaf.label)\cdot i$ is a prefix of both $val$ and $predLeaf.label$.
So, the $(|ancLeaf.label|+1)$th bit of $val$ and $predLeaf.label$ is $i$.
Since $predLeaf.label < leaf.label < val$, the $(|ancLeaf.label|+1)$th bit of $leaf$ is $i$.
So,  $(ancLeaf.label) \cdot i$ is a prefix of $leaf.label$ by Invariant \ref{prefix-inv}.

If $ancLeaf$ is $predAnc$, $ancLeaf.child[1]$ is visited at line \ref{predSearch-visit-node1} and $ancLeaf.child[0]$ is visited at line \ref{predSearch-visit-node2}.
So, $i$ could be 0 or 1.

If $(predAnc.label) \cdot 0$ is a prefix of $ancLeaf$, $ancChild$ is visited at line \ref{predSearch-visit-node1} and $i = 0$.
Since the condition at line \ref{predSearch-check-node} is satisfied for $ancLeaf$, $(ancLeaf.label)\cdot 0$ is a prefix of $val$.
Since $leaf.label < val$, $(ancLeaf.label)\cdot 0$ is a prefix of $leaf.label$.

If $(predAnc.label) \cdot 1$ is a prefix of $ancLeaf$, $ancChild$ is visited at line \ref{predSearch-visit-node3} and $i = 1$.
By Invarinat \ref{prefix-inv}, $(ancLeaf.label)\cdot 1$ is a prefix of $predLeaf.label$.
Since $predLeaf.label < leaf.label$, $(ancLeaf.label)\cdot 1$ is a prefix of $leaf.label$.

%If $i=0$, since $ancLeaf.label$ is a prefix of $leaf.label$ by Invariant \ref{prefix-inv} and $(ancLeaf.label) \cdot 0$ is a prefix of $predLeaf$ and $leaf.label < val$, $(|anc.label| + 1)$th bit of $val$ is $0$.
%If $i=1$, since $anc.label$ is a prefix of $leaf.label$ by Invariant \ref{prefix-inv} and $(anc.label) \cdot 1$ is a prefix of $preLeaf.label$ by Invariant \ref{prefix-inv} and $predLeaf.label < leaf.label$, 
%$(|anc.label| + 1)$th bit of $val$ is $1$.
Thus, $(ancLeaf.label) \cdot i$ is a prefix of $leaf.label$.
Since $ancLeaf$ is visited earlier at line \ref{predSearch-visit-node1}, \ref{predSearch-visit-node2} or \ref{predSearch-visit-node3}, 
$ancLeaf$ and $ancLeaf.child$ is stored in $result$ at line \ref{predSearch-set-result1}, \ref{predSearch-set-result2} or \ref{predSearch-set-result3}.
Since $ancLeaf$ is the lowest internal node that is visited before $predAnc$ and is unmarked at $T$, $anc$ is in $result$ when the operation returns.
By Lemma \ref{pred-no-child-change-lem}, $ancLeaf.child[i] = ancChild$ at $T$.
Since $ancLeaf$ is reachable at $T$, $ancChild$ is reachable at $T$.
By Lemma \ref{unreachable-flag-lem}, $ancChild$ is unmarked at $T$.
Since $ancLeaf$ is the lowest unmarked ancestor of $leaf$ at $T$, $ancChild$ is not an ancestor of $leaf$ at $T$.
Since $ancLeaf.child[i] = ancChild$ at $T$, $(|anc.label| + 1)$th bit of $leaf.label$ is $i$ and $ancChild$ is not ancestor of $leaf$ at $T$, $leaf$ is not reachable at $T$, contradicting that $leaf$ is logically in the trie at $T$.


Case 2: $node$ is an Internal node and  $node.label < |node.label|$ bits of $val$.
Let $anc$ be the lowest internal node that is unmarked at $T$, whose $label$ is a prefix of $predAnc.label$ and visited earlier at line \ref{predSearch-visit-node1} during the last call to the predSearch.
%(Since $root$ is never marked, such an ancestor exists at $T$.)
By Lemma \ref{unmarked-reachable-lem} and \ref{query-reachable-lem}, $anc$ is reachable at $T$. 

First, we show $anc$ is an ancestor of $leaf$ at $T$.
To derive a contradiction, assume $anc$ is not an ancestor of $leaf$ at $T$.
Since both $leaf$ and $anc$ are reachable at $T$, $anc.label$ is not a prefix of $leaf.label$.
Let $i$ be the leftmost bit of $anc.label$ that is different from that bit of $leaf.label$.
Note $node$ is the last node that is read at line \ref{predSearch-visit-node1} during the last call to the predSearch.
Since, at line \ref{predSearch-set-predAnc2}, $predAnc$ is set to a node whose child was $node$.
Since $anc.label$ is a prefix of $predAnc.label$, $anc.label$ is a prefix of $node.label$ by Invariant \ref{prefix-inv}.
Since the operation reads $predLeaf$ at line \ref{predSearch-visit-node3}, $node.label$ is a prefix of $predLeaf.label$ by Invariant \ref{prefix-inv}.
So, $anc.label$ is a prefix of $predLeaf.label$.
Since $predLeaf.label < leaf.label$ and $anc.label$ is a prefix of $predLeaf.label$, $i$th bit of $anc.label$ is 0.
Thus, $i$th bit of $leaf.label$ is 1.
Since $predAnc$ is not the last node that is visited at line \ref{predSearch-visit-node1}, the condition at line \ref{predSearch-check-node} for $predAnc$ is satisfied.
So, $predAnc.label$ is a prefix of $val$ and since $anc.label$ is a prefix of $predAnc.label$, $anc.label$ is a prefix of $val$.
Thus, $i$th bit of $val$ is 0, contradicting the fact that $leaf.label < val$ since $i$th bit of $leaf.label$ is 1. 

So, $anc$ is an ancestor of $leaf$ at $T$.
Let $ancLeaf$ be the lowest internal node whose $label$ is a prefix of $leaf.label$ and that is unmarked at $T$ and visited at line \ref{predSearch-visit-node1}, \ref{predSearch-visit-node2} or \ref{predSearch-visit-node3}.
(Since $anc$ exists, such an internal node exists.)
Let $ancChild$ be $ancLeaf.child[i]$ when it is visited earlier at line \ref{predSearch-visit-node1} during the predSearch.
%If $(|predAnc.label|+1)$th bit of $leaf.label$ is $0$, $ancLeaf$ is visited at line \ref{predSearch-visit-node1} after  $leaf.label < val$, 
%Then, $ancLeaf.label$ is a prefix of $predLeaf.label$ or $val$ or both.
Now, we show $(ancLeaf.label) \cdot i$ is a prefix of $leaf.label$.

Then, $ancLeaf$ is visited at line \ref{predSearch-visit-node1} before visiting $predAnc$ at line \ref{predSearch-visit-node1}. 
By Invariant \ref{prefix-inv}, since $predAnc.label$ is a prefix of both $val$ and $predLeaf.label$ and $(ancLeaf.label) \cdot i$ is a prefix of $predAnc.label$, 
$(ancLeaf.label)\cdot i$ is a prefix of both $val$ and $predLeaf.label$.
So, the $(|ancLeaf.label|+1)$th bit of $val$ and $predLeaf.label$ is $i$.
Since $predLeaf.label < leaf.label < val$, the $(|ancLeaf.label|+1)$th bit of $leaf$ is $i$.
So,  $(ancLeaf.label) \cdot i$ is a prefix of $leaf.label$ by Invariant \ref{prefix-inv}.

%Thus, $(ancLeaf.label) \cdot i$ is a prefix of $leaf.label$.
Since $ancLeaf$ is visited earlier at line \ref{predSearch-visit-node1} or \ref{predSearch-visit-node3}, 
$ancLeaf$ and $ancLeaf.child$ is stored in $result$ at line \ref{predSearch-set-result1}, \ref{predSearch-set-result2} or \ref{predSearch-set-result3}.
Since $ancLeaf$ is the lowest internal node that is visited before $predAnc$ and is unmarked at $T$, $ancLeaf$ is in $result$ when the operation returns.
By Lemma \ref{pred-no-child-change-lem}, $ancLeaf.child[i] = ancChild$ at $T$.
Since $ancLeaf$ is reachable at $T$, $ancChild$ is reachable at $T$.
By Lemma \ref{unreachable-flag-lem}, $ancChild$ is unmarked at $T$.
Since $ancLeaf$ is the lowest unmarked ancestor of $leaf$ at $T$, $ancChild$ is not an ancestor of $leaf$ at $T$.
Since $ancLeaf.child[i] = ancChild$ at $T$, $(|anc.label| + 1)$th bit of $leaf.label$ is $i$ and $ancChild$ is not ancestor of $leaf$ at $T$, $leaf$ is not reachable at $T$, contradicting that $leaf$ is logically in the trie at $T$.
\end{proof}

If the predecessor operation returns, it can be linearized at $T$ by Lemma \ref{pred-leaf-in-trie-lem}, \ref{pred-leaf-not-in-trie1-lem}, \ref{pred-leaf-not-in-trie2-lem}, and \ref{pred-leaf-not-in-trie3-lem}.
In Section \ref{correctness-update-sec}, we have shown that $activePoints$ is changed correctly just after the linearization points of update operations.
%In Section \ref{correctness-query-sec}, we showed that the query operations are linearized correctly.
Since $activePoints$ is changed correctly, the query operations return correct results at their linearization points.


